Out-of-Distribution Detection for LiDAR-based 3D Object Detection

3D object detection is an essential part of automated driving, and deep neural networks (DNNs) have achieved state-of-the-art performance for this task. However, deep models are notorious for assigning high confidence scores to out-of-distribution (OOD) inputs, that is, inputs that are not drawn from the training distribution. Detecting OOD inputs is challenging and essential for the safe deployment of models. OOD detection has been studied extensively for the classification task, but it has not received enough attention for the object detection task, specifically LiDAR-based 3D object detection. In this paper, we focus on the detection of OOD inputs for LiDAR-based 3D object detection. We formulate what OOD inputs mean for object detection and propose to adapt several OOD detection methods for object detection. We accomplish this by our proposed feature extraction method. To evaluate OOD detection methods, we develop a simple but effective technique of generating OOD objects for a given object detection model. Our evaluation based on the KITTI dataset shows that different OOD detection methods have biases toward detecting specific OOD objects. It emphasizes the importance of combined OOD detection methods and more research in this direction.

==> fig/base_fp_seed_10.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_fp_seed_10.png}
\end{center}
\caption{
% 
OOD base fp 10
}
\label{fig:base_fp_10}
\end{figure*}

==> fig/base_seed_10.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_carla_seed_10.png}
\end{center}
\caption{
% 
OOD base carla 10
}
\label{fig:base_carla_10}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_fp_seed_10.png}
\end{center}
\caption{
% 
OOD base fp 10
}
\label{fig:base_fp_10}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_waymo_seed_10.png}
\end{center}
\caption{
% 
OOD base waymo 10
}
\label{fig:base_waymo_10}
\end{figure*}

==> fig/base_seed_14.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_carla_seed_14.png}
\end{center}
\caption{
% 
OOD base carla 14
}
\label{fig:base_carla_14}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_fp_seed_14.png}
\end{center}
\caption{
% 
OOD base fp 14
}
\label{fig:base_fp_14}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_waymo_seed_14.png}
\end{center}
\caption{
% 
OOD base waymo 14
}
\label{fig:base_waymo_14}
\end{figure*}

==> fig/base_seed_17.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_carla_seed_17.png}
\end{center}
\caption{
% 
OOD base carla 17
}
\label{fig:base_carla_17}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_fp_seed_17.png}
\end{center}
\caption{
% 
OOD base fp 17
}
\label{fig:base_fp_17}
\end{figure*}

\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_waymo_seed_17.png}
\end{center}
\caption{
% 
OOD base waymo 17
}
\label{fig:base_waymo_17}
\end{figure*}

==> fig/base_waymo_17.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_waymo_seed_10.png}
\end{center}
\caption{
% 
OOD base waymo 10
}
\label{fig:base_waymo_10}
\end{figure*}

==> fig/base_waymo_seed_10.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/base_waymo_seed_10.png}
\end{center}
\caption{
% 
OOD base waymo 10
}
\label{fig:base_waymo_10}
\end{figure*}

==> fig/objects_scenes.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.8\linewidth]{fig/object_scenes.png}
\end{center}
\caption{
% 
Examples of Carla objects in red circle inserted in scenes 
}
\label{fig:object_scenes}
\end{figure}

==> fig/ood-venn.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\textwidth]{fig/ood-venn-diagram.png}
\end{center}
\caption{
% 
OOD diagram
}
\label{fig:ood-venn-diagram}
\end{figure}


==> fig/ood_gen_diagram.tex <==
\begin{figure*}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.8\textwidth]{fig/ood_dataset_generation.pdf}
\end{center}
\caption{
% 
OOD dataset generation diagram
}
\label{fig:ood_gen_diagram}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=\linewidth]{example-image-golden}
\end{center}
\caption{
% 
\textbf{Teaser -- }
Some nice summarizing image.
}
\label{fig:teaser}
\end{figure}

==> tab/all_carla_database.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c|c}
\toprule
Class &   Quantity \\
\midrule
ATM  & 10\\
\midrule
Bench  & 44\\
\midrule
Swing couch  & 25\\
\midrule
Trash can 1  & 5\\
\midrule
Trash can 2  & 5\\
\midrule
Plant  & 5\\
\midrule
Park light &  5\\
\bottomrule
\end{tabular}
\caption{The number of objects per class in  Carla OOD database}
\label{tab:all_carla_database}
\end{table}


==> tab/all_fp_database.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c|c}
\toprule
Class &   Quantity \\
\midrule
Sidewalk sign &  33 \\
\midrule
Bike rack & 11 \\
\midrule
Low traffic sign & 10 \\
\midrule
Potted plan & 9\\
\midrule
Thin sign & 3 \\
\midrule
Tree & 2 \\
\midrule
Product rack & 2 \\
\midrule
Back of a car & 2 \\
\bottomrule
\end{tabular}
\caption{The number of objects per class in KITTI FP OOD database}
\label{tab:all_fp_database}
\end{table}


% Sidewalk sign 33
% Bike rack 11
% Low traffic sign 10
% Potted plan 9
% Thin sign 3
% Tree 2
% Product rack 2
% Back of a car 2





==> tab/all_results.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{fig/common_ood.pdf}
%     \caption{The distribution of OOD objects detected by both base model and contrastive model}
%     \label{fig:common_ood}
% \end{figure}

\begin{table}
    \centering
    \tiny
    \begin{tabular}{rc|ccc|ccc}
    \toprule
                      &     & \multicolumn{3}{c}{AUROC $\uparrow$} & \multicolumn{3}{c}{FPR @ 95 TPR $\downarrow$} \\
    \textbf{OOD Method} & \textbf{Layer} & Base &  Ctrst & $\Delta$ &          Base &  Ctrst & $\Delta$ \\
    \midrule
    \textbf{Max Softmax} & \textbf{-} &  89.95 &  \underline{\textbf{89.97}} &    \textbf{ 0.02} &          33.83 &  \underline{\textbf{31.86}} &   \textbf{ -1.97} \\
    \textbf{Predictive Entropy} & \textbf{-} &  83.49 &  84.80 &     \textbf{1.32} &          39.60 &  34.54 &   \textbf{ -5.05} \\
    \textbf{Aleatoric Entropy} & \textbf{-} &  83.09 &  84.65 &     \textbf{1.56} &          41.77 &  36.41 &   \textbf{ -5.37} \\
    \textbf{Mutual Information} & \textbf{-} &  60.48 &  60.70 &     \textbf{0.23} &          97.07 &  96.51 &    \textbf{-0.56} \\
    \textbf{Mahalanobis} & \textbf{backbone} &  83.77 &  84.56 &     \textbf{0.80} &          51.01 &  43.92 &    \textbf{-7.10} \\
    \textbf{OCSVM} & \textbf{conv8x} &  65.44 &  62.91 &    -2.53 &          66.20 &  70.31 &     4.11 \\
    \textbf{RealNVP} & \textbf{backbone} & \underline{ \textbf{90.28}} &  88.30 &    -1.98 &          \underline{\textbf{26.72}} &  33.14 &     6.42 \\
    \bottomrule
    \end{tabular}

    \caption{The OOD detection results for all OOD objects such that each detected by both models. For each metric, we underline the best performing OOD method. We also show the performance difference $\Delta$ between contrastive model and base model, with bold numbers indicating contrastive model has better performance. All results are averaged over three sets of experiments.}
    \label{tab:results_all}
\end{table}

\begin{table}
    \tiny
    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{rc|ccc|ccc}
        \toprule
                          &     & \multicolumn{3}{c}{AUROC $\uparrow$} & \multicolumn{3}{c}{FPR @ 95 TPR $\downarrow$} \\
        \textbf{OOD Method} & \textbf{Layer} & Base &  Ctrst & $\Delta$ &          Base &  Ctrst & $\Delta$ \\
        \midrule
        \textbf{Max Softmax} & \textbf{-} &  \underline{\textbf{96.04}} &  \underline{\textbf{96.15}} &     \textbf{0.11} &          \underline{\textbf{10.39}} &  \underline{\textbf{10.23}} &    \textbf{-0.16} \\
        \textbf{Predictive Entropy} & \textbf{-} &  85.34 &  87.12 &     \textbf{1.78} &          35.55 &  30.10 &    \textbf{-5.45} \\
        \textbf{Aleatoric Entropy} & \textbf{-} &  85.30 &  87.37 &     \textbf{2.06} &          37.87 &  30.76 &    \textbf{-7.11} \\
        \textbf{Mutual Information} & \textbf{-} &  45.04 &  43.18 &    -1.86 &          98.75 &  98.66 &    \textbf{-0.09} \\
        \textbf{Mahalanobis} & \textbf{backbone} &  88.34 &  89.88 &     \textbf{1.54} &          37.49 &  35.78 &    \textbf{-1.71} \\
        \textbf{OCSVM} & \textbf{conv8x} &  66.49 &  63.12 &    -3.37 &          63.49 &  70.01 &     6.53 \\
        \textbf{RealNVP} & \textbf{backbone} &  93.63 &  92.50 &    -1.13 &          19.90 &  22.80 &     2.90 \\
        \bottomrule
        \end{tabular}
    
        \caption{Carla}
        \label{tab:results_carla}
    \end{subtable}
    
    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{rc|ccc|ccc}
        \toprule
                          &     & \multicolumn{3}{c}{AUROC $\uparrow$} & \multicolumn{3}{c}{FPR @ 95 TPR $\downarrow$} \\
        \textbf{OOD Method} & \textbf{Layer} & Base &  Ctrst & $\Delta$ &          Base &  Ctrst & $\Delta$ \\
        \midrule
        \textbf{Max Softmax} & \textbf{-} & \underline{\textbf{95.58}} &  \underline{\textbf{96.06}} &     \textbf{0.48} &          \underline{\textbf{21.23}} &  \underline{\textbf{20.80}} &    \textbf{-0.43} \\
        \textbf{Predictive Entropy} & \textbf{-} &  78.65 &  80.41 &     \textbf{1.76} &          41.66 &  36.10 &    \textbf{-5.55} \\
        \textbf{Aleatoric Entropy} & \textbf{-} &  78.24 &  80.03 &     \textbf{1.79} &          43.93 &  38.59 &    \textbf{-5.33} \\
        \textbf{Mutual Information} & \textbf{-} &  52.09 &  55.94 &     \textbf{3.86} &          99.13 &  98.58 &    \textbf{-0.55} \\
        \textbf{Mahalanobis} & \textbf{backbone} &  86.25 &  84.09 &    -2.16 &          54.35 &  50.86 &    \textbf{-3.48} \\
        \textbf{OCSVM} & \textbf{conv8x} &  66.95 &  63.67 &    -3.28 &          62.58 &  69.03 &     6.45 \\
        \textbf{RealNVP} & \textbf{backbone} &  85.81 &  84.02 &    -1.79 &          31.17 &  32.49 &     1.31 \\
        \bottomrule
        \end{tabular}
    
        \caption{KITTI Ignored}
        \label{tab:results_ignored}
    \end{subtable}
    
    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{rc|ccc|ccc}
        \toprule
                          &     & \multicolumn{3}{c}{AUROC $\uparrow$} & \multicolumn{3}{c}{FPR @ 95 TPR $\downarrow$} \\
        \textbf{OOD Method} & \textbf{Layer} & Base &  Ctrst & $\Delta$ &          Base &  Ctrst & $\Delta$ \\
        \midrule
        \textbf{Max Softmax} & \textbf{-} &  82.84 &  82.87 &     \textbf{0.03} &          36.41 &  34.05 &    \textbf{-2.36} \\
        \textbf{Predictive Entropy} & \textbf{-} &  86.92 &  86.76 &    -0.16 &          29.69 &  27.96 &    \textbf{-1.73} \\
        \textbf{Aleatoric Entropy} & \textbf{-} &  86.76 &  86.77 &     \textbf{0.02} &          30.09 &  28.24 &    \textbf{-1.86} \\
        \textbf{Mutual Information} & \textbf{-} &  70.62 &  72.47 &     \textbf{1.86} &          85.78 &  82.66 &    \textbf{-3.12} \\
        \textbf{Mahalanobis} & \textbf{backbone} &  72.48 &  80.60 &     \textbf{8.11} &          59.52 &  38.05 &   \textbf{-21.47} \\
        \textbf{OCSVM} & \textbf{conv8x} &  63.22 &  62.59 &    -0.63 &          72.03 &  70.91 &    \textbf{-1.11} \\
        \textbf{RealNVP} & \textbf{backbone} &  \underline{\textbf{91.71}} &  \underline{\textbf{91.81}} &     \textbf{0.10} &          \underline{\textbf{16.25}} &  \underline{\textbf{15.44}} &    \textbf{-0.81} \\
        \bottomrule
        \end{tabular}
    
        \caption{KITTI FP}
        \label{tab:results_fp}
    \end{subtable}
    
    \begin{subtable}{\linewidth}
        \centering
        \begin{tabular}{rc|ccc|ccc}
        \toprule
                          &     & \multicolumn{3}{c}{AUROC $\uparrow$} & \multicolumn{3}{c}{FPR @ 95 TPR $\downarrow$} \\
        \textbf{OOD Method} & \textbf{Layer} & Base &  Ctrst & $\Delta$ &          Base &  Ctrst & $\Delta$ \\
        \midrule
        \textbf{Max Softmax} & \textbf{-} &  83.18 &  \underline{\textbf{83.34}} &     \textbf{0.16} &          52.17 &  \underline{\textbf{45.80}} &    \textbf{-6.36} \\
        \textbf{Predictive Entropy} & \textbf{-} &  80.64 &  81.23 &     \textbf{0.58} &          53.69 &  47.50 &    \textbf{-6.19} \\
        \textbf{Aleatoric Entropy} & \textbf{-} &  80.01 &  80.90 &     \textbf{0.88} &          53.97 &  47.62 &    \textbf{-6.36} \\
        \textbf{Mutual Information} & \textbf{-} &  67.53 &  66.41 &    -1.12 &          90.14 &  86.23 &    \textbf{-3.91} \\
        \textbf{Mahalanobis} & \textbf{backbone} &  \underline{\textbf{88.30}} &  82.21 &    -6.09 &          43.53 &  51.34 &     7.80 \\
        \textbf{OCSVM} & \textbf{conv8x} &  64.74 &  62.20 &    -2.55 &          67.81 &  71.51 &     3.70 \\
        \textbf{RealNVP} & \textbf{backbone} &  85.44 &  79.56 &    -5.88 &          \underline{\textbf{33.03}} &  46.01 &    12.98 \\
        \bottomrule
        \end{tabular}
    
        \caption{Waymo}
        \label{tab:results_waymo}
    \end{subtable}
    
    \caption{The OOD detection results for OOD object datasets.}
    \label{tab:results_type}
\end{table}


==> tab/all_waymo_database.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c|c}
\toprule
Class &   Quantity \\
\midrule
Boom truck  & 20 \\
\midrule
Box truck  & 161 \\
\midrule
Digger  & 49 \\
\midrule
Cement truck   &26 \\
\midrule
Trailer  & 134 \\
\midrule
Pickup truck  & 922 \\
\midrule
Mobile traffic sign  & 24 \\
\midrule
Semi truck  & 193 \\
\midrule
Transit bus & 407 \\
\midrule
Motorcycle  & 456 \\
\midrule
Flatbed truck  & 220 \\
\midrule
Scooter  & 80 \\
\midrule
Garbage truck  & 20 \\
\midrule
Greyhound bus  & 173 \\
\midrule
Dump truck  & 37 \\
\midrule
Excavator  & 44 \\
\midrule
Tow truck   & 8 \\
\midrule
Boat trailer  & 14 \\
\midrule
Lorry  & 51 \\
\midrule
Bucket truck  & 30 \\
\midrule
RV  & 40 \\
\midrule
Construction truck  & 8 \\
\midrule
Mail truck  & 65 \\
\midrule
Food truck  & 9 \\
\midrule
Boom lift  & 20 \\
\midrule
Boat  & 10\\
\midrule
Camper  &  20\\
\midrule
Modified motor tricycle & 7 \\
\bottomrule
\end{tabular}
\caption{The number of objects per class in  Waymo OOD database}
\label{tab:all_waymo_database}
\end{table}

% boom_truck 20
% box_truck 161
% digger 49
% cement_truck 26
% trailer 134
% pickup_truck 922
% mobile_traffic_sign 24
% semi_truck 193
% transit_bus 407
% motorcycle 456
% flatbed_truck 220
% scooter 80
% garbage_truck 20
% greyhound_bus 173
% dump_truck 37
% excavator 44
% tow_truck 8
% boat_trailer 14
% lorry 51
% bucket_truck 30
% RV 40
% construction_truck 8
% mail_truck 65
% food_truck 9
% boom_lift 20
% boat 10
% camper 20
% modified_motor_tricycle 7

==> tab/carla_adding_statistics.tex <==
\begin{table}
\centering
\tiny
\begin{tabular}{c|ccc}
\toprule
Class & Adding failures & Detecting failures & Number of attempted frames \\
\midrule
ATM  & 16.86 & 41.91& 525 \\
\midrule
Bench  & 24.23 &  60.18& 1903       \\
\midrule
Swing couch  & 26.06 & 52.30 &1590 \\
\midrule
Trash can 01 & 17.51 & 46.10 & 577   \\
\midrule
Trash can 02 & 3.47 & 8.02 &304  \\
\bottomrule
\end{tabular}
\caption{Carla inserting statistics}
\label{tab:carla_inserting_statistics}
\end{table}



==> tab/carla_database.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{c|cccccc}
\toprule
Class &   ATM &  Bench & Swing couch & Trash can 1 & Trash can 2 \\
\midrule
Quantity  & 10 &  44 & 25 & 5 & 5 \\
\bottomrule
\end{tabular}
\caption{The number of objects per selected class in  Carla OOD database}
\label{tab:carla_database}
\end{table}

==> tab/fp_adding_statistics.tex <==
\begin{table}
\centering
\tiny
\begin{tabular}{c|ccc}
\toprule
Class & Adding failures & Detecting failures & Number of attempted frames \\
\midrule
Bike rack  & 0.82 &  0.06 & 300 \\
\midrule
Potted plant  & 0.79 & 0.03  & 300  \\
\midrule
Sidewalk sign  & 0.47 &  0.01& 300 \\
\midrule
Low traffic sign & 0.27  & 0.02& 300  \\
\midrule
Thin sign & 0.45 &  0.07 & 300    \\
\bottomrule
\end{tabular}
\caption{KITTI FP inserting statistics}
\label{tab:fp_inserting_statistics}
\end{table}

% bike_rack
% [  0.822   0.064 300.   ]
% potted_plant
% [  0.797   0.03  300.   ]
% sidewalk_sign
% [  0.473   0.014 300.   ]
% low_traffic_sign
% [  0.274   0.019 300.   ]
% thin_sign
% [  0.452   0.072 300.   ]

==> tab/fp_database_base_10.tex <==
\begin{table}
\centering
\tiny
\begin{tabular}{c|ccccc}
\toprule
Class &   Bike rack & Sidewalk sign & Traffic sign & Potted plant & Thin sign \\
\midrule
Quantity  & 11 &  33 & 10 & 9 & 3\\
\bottomrule
\end{tabular}
\caption{The number of objects per selected class in  KITTI FP OOD database}
\label{tab:fp_database}
\end{table}



==> tab/fp_training_stats.tex <==
\begin{table}[H]
\centering
\tiny
\begin{tabular}{c|ccccc}
\toprule
Class &   Bike rack & Sidewalk sign & Traffic sign & Potted plant & Thin sign \\
\midrule
Quantity  & 0 &  625 & 295 & 298 & 60\\
\bottomrule
\end{tabular}
\caption{The number of times that KITTI FP objects appear in the KITTI training dataset}
\label{tab:fp-in-training}
\end{table}

==> tab/full_results.tex <==
\begin{table*}
\centering
\tiny
\begin{tabular}{rc|ccc|ccc|ccc|ccc|ccc}
\toprule
        &       & \multicolumn{3}{c}{AUROC} & \multicolumn{3}{c}{AUPR (ID)} & \multicolumn{3}{c}{AUPR (OOD)} & \multicolumn{3}{c}{FPR @ 95\% TPR} & \multicolumn{3}{c}{Detection Err.} \\
       \textbf{OOD Method} &    \textbf{Layer}   &   Base &  Ctrst & $\Delta$ &      Base &  Ctrst & $\Delta$ &       Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ \\
\midrule
\textbf{Max Softmax} & \textbf{-} &  89.95 &  \underline{\textbf{89.97}} &     \textbf{0.02} &     91.46 &  \underline{\textbf{91.85}} &     \textbf{0.38} &      \underline{\textbf{88.01}} &  \underline{\textbf{87.66}} &    -0.35 &          33.83 &  \underline{\textbf{31.86}} &    \textbf{-1.97} &          19.33 &  \underline{\textbf{18.32}} &    \textbf{-1.00} \\
\textbf{Predictive Entropy} & \textbf{-} &  83.49 &  84.80 &     \textbf{1.32} &     87.50 &  88.94 &     \textbf{1.44} &      76.48 &  77.56 &     \textbf{1.08} &          39.60 &  34.54 &    \textbf{-5.05} &          22.19 &  19.65 &    \textbf{-2.54} \\
\textbf{Aleatoric Entropy} & \textbf{-} &  83.09 &  84.65 &     \textbf{1.56} &     87.03 &  88.67 &     \textbf{1.64} &      75.93 &  77.75 &     \textbf{1.82} &          41.77 &  36.41 &    \textbf{-5.37} &          23.29 &  20.57 &    \textbf{-2.71} \\
\textbf{Mutual Information} & \textbf{-} &  60.48 &  60.70 &     \textbf{0.23} &     54.10 &  54.79 &     \textbf{0.69} &      64.48 &  63.87 &    -0.61 &          97.07 &  96.51 &    \textbf{-0.56} &          49.98 &  49.83 &    \textbf{-0.15} \\
\midrule
\multirow{6}{*}{\textbf{Mahalanobis}} & \textbf{logits} &  66.55 &  67.76 &     \textbf{1.21} &     59.28 &  59.04 &    -0.25 &      71.47 &  72.36 &     \textbf{0.88} &          93.81 &  95.31 &     1.51 &          49.16 &  49.70 &     0.54 \\
        & \textbf{backbone} &  \textbf{83.77} &  \textbf{84.56} &     \textbf{0.80} &     \textbf{85.30} &  \textbf{86.73} &     \textbf{1.43} &      \textbf{81.65} &  \textbf{81.93} &     \textbf{0.28} &          \textbf{51.01} &  \textbf{43.92} &   \textbf{-7.10} &          \textbf{27.89} &  \textbf{24.34} &    \textbf{-3.55} \\
        & \textbf{conv2x} &  79.37 &  79.48 &     \textbf{0.11} &     78.46 &  77.89 &    -0.56 &      77.93 &  78.78 &     \textbf{0.85} &          70.36 &  72.44 &     2.07 &          37.55 &  38.55 &     1.00 \\
        & \textbf{conv4x} &  66.94 &  69.12 &     \textbf{2.18} &     64.28 &  66.95 &     \textbf{2.67} &      66.12 &  67.91 &     \textbf{1.79} &          87.43 &  83.99 &    \textbf{-3.44} &          46.11 &  44.41 &    \textbf{-1.70} \\
        & \textbf{conv8x} &  62.71 &  68.68 &     \textbf{5.97} &     60.76 &  69.02 &     \textbf{8.26} &      59.53 &  64.91 &     \textbf{5.38} &          90.34 &  79.83 &   \textbf{-10.51} &          47.55 &  42.32 &   \textbf{-5.23} \\
        & \textbf{ctrst} &    - &  74.89 &      - &       - &  68.37 &      - &        - &  76.07 &      - &            - &  87.09 &      - &            - &  45.91 &      - \\
\midrule
\multirow{5}{*}{\textbf{OCSVM}} & \textbf{logits} &  52.53 &  46.45 &    -6.08 &     51.69 &  45.98 &    -5.71 &      57.43 &  54.11 &    -3.32 &          93.75 &  97.78 &     4.03 &          48.16 &  49.96 &     1.79 \\
        & \textbf{conv2x} &  60.28 &  61.47 &     \textbf{1.19} &     68.82 &  69.42 &     \textbf{0.60} &      75.62 &  75.94 &     \textbf{0.32} &          79.80 &  80.28 &     0.48 &          42.25 &  42.53 &     0.28 \\
        & \textbf{conv4x} &  51.38 &  52.51 &     \textbf{1.13} &     49.92 &  50.93 &     \textbf{1.02} &      70.07 &  70.58 &     \textbf{0.51} &          97.95 &  97.94 &    \textbf{-0.01} &          49.97 &  49.95 &    \textbf{-0.02} \\
        & \textbf{conv8x} &  \textbf{65.44} &  \textbf{62.91} &    -2.53 &    \textbf{ 78.76} &  \textbf{79.93} &     \textbf{1.17} &      \textbf{78.83} &  \textbf{78.54} &    -0.29 &         \textbf{ 66.20} &  \textbf{70.31} &     4.11 &          \textbf{35.31} &  \textbf{37.17} &     1.86 \\
        & \textbf{ctrst} &    - &  58.58 &      - &       - &  49.88 &      - &        - &  70.75 &      - &            - &  98.15 &      - &            - &  49.99 &      - \\
\midrule
\multirow{6}{*}{\textbf{RealNVP}} & \textbf{logits} &  63.84 &  61.46 &    -2.38 &     61.93 &  60.33 &    -1.59 &      63.24 &  60.20 &    -3.04 &          88.02 &  89.11 &     1.09 &          46.38 &  46.83 &     0.46 \\
        & \textbf{backbone} & \underline{\textbf{90.28}}&  88.30 &    -1.98 &     \underline{\textbf{92.67}} &  \textbf{90.89} &    -1.78 &     \textbf{ 86.93} &  \textbf{84.72} &    -2.21 &         \underline{\textbf{26.72}} &  33.14 &     6.42 &          \underline{\textbf{15.72}} &  18.97 &     3.25 \\
        & \textbf{conv2x} &  78.09 &  83.64 &     \textbf{5.56} &     76.87 &  84.42 &     \textbf{7.56} &      78.58 &  81.57 &     \textbf{2.99} &          66.04 &  51.86 &   \textbf{-14.18} &          35.34 &  28.33 &    \textbf{-7.01} \\
        & \textbf{conv4x} &  87.56 &  \textbf{88.41} &     \textbf{0.85} &     88.52 &  89.66 &     \textbf{1.15} &      86.61 &  86.27 &    -0.33 &          48.26 &  41.69 &    \textbf{-6.57} &          26.52 &  23.16 &    \textbf{-3.36} \\
        & \textbf{ctrst} &    - &  87.32 &      - &       - &  89.38 &      - &        - &  83.19 &      - &            - &  \textbf{32.95} &      - &            - &  \textbf{18.89} &      - \\
\bottomrule
\end{tabular}
\caption{Results for all common OOD objects detected by both base and contrastive models. For Mahalanobis distance, OC-SVM, and RealNVP, we bold the best performing layer for each method. The best performing OOD method/layer for each metric is underlined. We also report the difference $\Delta$ between contrastive model and base model, with bold numbers indicating contrastive model has better performance. All results are averaged over three sets of experiments.}
\label{tab:full_results_all}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{rc|ccc|ccc|ccc|ccc|ccc}
\toprule
        &       & \multicolumn{3}{c}{AUROC} & \multicolumn{3}{c}{AUPR (ID)} & \multicolumn{3}{c}{AUPR (OOD)} & \multicolumn{3}{c}{FPR @ 95\% TPR} & \multicolumn{3}{c}{Detection Err.} \\
       \textbf{OOD Method} &    \textbf{Layer}   &   Base &  Ctrst & $\Delta$ &      Base &  Ctrst & $\Delta$ &       Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ \\
\midrule
\textbf{Max Softmax} & \textbf{-} &  \underline{\textbf{96.04}} &  \underline{\textbf{96.15}} &     \textbf{0.11} &    \underline{\textbf{97.25}} &  \underline{\textbf{97.35}} &     \textbf{0.11} &      \underline{\textbf{93.46}} &  \underline{\textbf{93.45}} &    -0.02 &          \underline{\textbf{10.39}} &  \underline{\textbf{10.23}} &    \textbf{-0.16} &           \underline{\textbf{7.39}} &   \underline{\textbf{7.28}} &    \textbf{-0.11} \\
\textbf{Predictive Entropy} & \textbf{-} &  85.34 &  87.12 &     \textbf{1.78} &     89.42 &  91.06 &     \textbf{1.64} &      77.72 &  79.29 &     \textbf{1.58} &          35.55 &  30.10 &    \textbf{-5.45} &          20.15 &  17.22 &    \textbf{-2.92} \\
\textbf{Aleatoric Entropy} & \textbf{-} &  85.30 &  87.37 &     \textbf{2.06} &     89.07 &  90.98 &     \textbf{1.91} &      77.99 &  80.25 &     \textbf{2.26} &          37.87 &  30.76 &    \textbf{-7.11} &          21.34 &  17.69 &    \textbf{-3.65} \\
\textbf{Mutual Information} & \textbf{-} &  45.04 &  43.18 &    -1.86 &     44.13 &  43.54 &    -0.59 &      53.30 &  50.95 &    -2.35 &          98.75 &  98.66 &    \textbf{-0.09} &          49.99 &  49.99 &    -0.00 \\
\midrule
\multirow{6}{*}{\textbf{Mahalanobis}} & \textbf{logits} &  83.51 &  83.40 &    -0.11 &     81.04 &  80.53 &    -0.51 &      84.63 &  83.31 &    -1.32 &          66.26 &  69.77 &     3.51 &          35.55 &  37.31 &     1.75 \\
        & \textbf{backbone} &  \textbf{88.34} &  \textbf{89.88} &     \textbf{1.54} &     \textbf{89.99} &  \textbf{90.86} &     \textbf{0.87} &      \textbf{86.44} &  88.35 &     \textbf{1.90} &          \textbf{37.49} &  35.78 &    \textbf{-1.71} &          \textbf{21.16} &  20.29 &    \textbf{-0.87} \\
        & \textbf{conv2x} &  85.82 &  88.80 &     \textbf{2.98} &     84.44 &  85.90 &    \textbf{1.45} &      85.10 &  \textbf{89.61} &     \textbf{4.50} &          53.82 &  58.01 &     4.19 &          29.35 &  31.44 &     2.09 \\
        & \textbf{conv4x} &  72.57 &  80.11 &     \textbf{7.53} &     73.83 &  81.42 &     \textbf{7.60} &      68.86 &  77.10 &     \textbf{8.24} &          72.85 &  60.14 &   \textbf{-12.71} &          38.83 &  32.49 &    \textbf{-6.34} \\
        & \textbf{conv8x} &  67.08 &  71.82 &     \textbf{4.75} &     71.95 &  75.88 &     \textbf{3.93} &      58.73 &  63.58 &     \textbf{4.85} &          70.17 &  63.25 &    \textbf{-6.91} &          37.49 &  34.02 &    \textbf{-3.47} \\
        & \textbf{ctrst} &    - &  89.81 &      - &       - &  90.19 &      - &        - &  85.08 &      - &            - &  \textbf{35.07} &      - &            - &  \textbf{19.95} &      - \\
\midrule
\multirow{5}{*}{\textbf{OC-SVM}} & \textbf{logits} &  54.26 &  48.41 &    -5.85 &     51.69 &  47.02 &    -4.67 &      58.74 &  56.45 &    -2.29 &          96.38 &  97.57 &     1.19 &          49.53 &  49.84 &     0.31 \\
        & \textbf{conv2x} &  63.61 &  64.82 &     \textbf{1.21} &     77.11 &  76.76 &    -0.34 &      78.39 &  78.60 &     \textbf{0.22} &          68.39 &  \textbf{66.22} &    \textbf{-2.17} &          36.37 &  \textbf{35.43} &    \textbf{-0.94} \\
        & \textbf{conv4x} &  61.50 &  63.16 &     \textbf{1.66} &     74.71 &  76.27 &     \textbf{1.56} &      77.47 &  78.16 &     \textbf{0.69} &          77.32 &  71.20 &    \textbf{-6.12} &          40.91 &  37.92 &    \textbf{-2.99} \\
        & \textbf{conv8x} &  \textbf{66.49} &  63.12 &    -3.37 &     \textbf{82.29} &  \textbf{80.74} &    -1.55 &      \textbf{79.78} &  78.74 &    -1.04 &          \textbf{63.49} &  70.01 &     6.53 &          \textbf{33.61} &  36.92 &     3.30 \\
        & \textbf{ctrst} &    - &  \textbf{72.38} &      - &       - &  62.21 &      - &        - &  \textbf{79.69} &      - &            - &  93.43 &      - &            - &  48.82 &      - \\
\midrule
\multirow{6}{*}{\textbf{RealNVP}} & \textbf{logits} &  70.81 &  70.26 &    -0.55 &     74.09 &  73.57 &    -0.52 &      66.90 &  65.64 &    -1.26 &          68.84 &  69.44 &     0.60 &          36.82 &  37.10 &     0.28 \\
        & \textbf{backbone} &  93.63 &  92.50 &    -1.13 &     95.16 &  94.17 &    -0.99 &      90.82 &  89.22 &    -1.59 &          19.90 &  22.80 &     2.90 &          12.11 &  13.75 &     1.64 \\
        & \textbf{conv2x} &  92.07 &  93.59 &     \textbf{1.51} &     92.03 &  93.05 &     \textbf{1.03} &      91.43 &  92.66 &     \textbf{1.22} &          24.79 &  21.81 &    \textbf{-2.98} &          14.79 &  13.32 &   \textbf{-1.47} \\
        & \textbf{conv4x} &  \textbf{94.65} &  \textbf{95.79} &     \textbf{1.13} &     \textbf{95.92} &  \textbf{97.01} &     \textbf{1.09} &      \textbf{92.25} &  \textbf{92.78} &     \textbf{0.53} &          \textbf{17.85} &  \textbf{12.24} &    \textbf{-5.61} &          \textbf{11.12} &   \textbf{8.22} &    \textbf{-2.90} \\
        & \textbf{conv8x} &  88.96 &  84.02 &    -4.94 &     92.13 &  87.70 &    -4.42 &      80.85 &  76.57 &    -4.28 &          26.83 &  39.55 &    12.71 &          15.81 &  22.15 &     6.33 \\
        & \textbf{ctrst} &    - &  92.44 &      - &       - &  94.78 &      - &        - &  87.81 &      - &            - &  16.66 &      - &            - &  10.52 &      - \\
\bottomrule
\end{tabular}
\caption{Results for Carla objects}
\label{tab:full_results_carla}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{rc|ccc|ccc|ccc|ccc|ccc}
\toprule
        &       & \multicolumn{3}{c}{AUROC} & \multicolumn{3}{c}{AUPR (ID)} & \multicolumn{3}{c}{AUPR (OOD)} & \multicolumn{3}{c}{FPR @ 95\% TPR} & \multicolumn{3}{c}{Detection Err.} \\
       \textbf{OOD Method} &    \textbf{Layer}   &   Base &  Ctrst & $\Delta$ &      Base &  Ctrst & $\Delta$ &       Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ \\
\midrule
\textbf{Max Softmax} & \textbf{-} &  \underline{\textbf{95.38}} &  \underline{\textbf{96.06}} &     \textbf{0.48} &     \underline{\textbf{95.80}} &  \underline{\textbf{96.35}} &     \textbf{0.55} &      \underline{\textbf{95.32}} &  \underline{\textbf{95.77}} &     \textbf{0.45} &          \underline{\textbf{21.23}} &  \underline{\textbf{20.80}} &    \textbf{-0.43} &          \underline{\textbf{12.34}} &  \underline{\textbf{12.27}} &    \textbf{-0.08} \\
\textbf{Predictive Entropy} & \textbf{-} &  78.65 &  80.41 &     \textbf{1.76} &     84.83 &  86.59 &     \textbf{1.76} &      69.75 &  71.44 &     \textbf{1.69} &          41.66 &  36.10 &    \textbf{-5.55} &          22.74 &  20.01 &    \textbf{-2.73} \\
\textbf{Aleatoric Entropy} & \textbf{-} &  78.24 &  80.03 &     \textbf{1.79} &     84.31 &  86.11 &     \textbf{1.80} &      69.29 &  71.30 &     \textbf{2.01} &          43.93 &  38.59 &    \textbf{-5.33} &          24.00 &  21.26 &    \textbf{-2.73} \\
\textbf{Mutual Information} & \textbf{-} &  52.09 &  55.94 &     \textbf{3.86} &     47.53 &  50.16 &     \textbf{2.63} &      60.33 &  63.24 &     \textbf{2.91} &          99.13 &  98.58 &    \textbf{-0.55} &          49.95 &  49.96 &     0.01 \\
\midrule
\multirow{6}{*}{\textbf{Mahalanobis}} & \textbf{logits} &  74.12 &  78.08 &     \textbf{3.96} &     68.50 &  75.29 &     \textbf{6.79} &      73.93 &  75.74 &     \textbf{1.80} &          88.34 &  78.49 &    \textbf{-9.85} &          45.92 &  41.11 &    \textbf{-4.82} \\
        & \textbf{backbone} &  \textbf{86.25} &  84.09 &    -2.16 &     \textbf{86.07} &  85.46 &    -0.61 &      \textbf{85.98} &  83.46 &    -2.52 &          54.35 &  50.86 &    \textbf{-3.48} &          \textbf{28.80} &  27.18 &    \textbf{-1.62} \\
        & \textbf{conv2x} &  63.77 &  59.44 &    -4.33 &     62.04 &  59.80 &    -2.25 &      65.70 &  58.77 &    -6.93 &          90.77 &  88.91 &    \textbf{-1.86} &          46.81 &  46.23 &    \textbf{-0.58} \\
        & \textbf{conv4x} &  72.09 &  69.64 &    -2.44 &     70.67 &  67.15 &    -3.52 &      72.15 &  67.54 &    -4.62 &          78.82 &  84.29 &     5.47 &          41.25 &  43.94 &     2.68 \\
        & \textbf{conv8x} &  85.02 &  89.98 &     \textbf{4.96} &     84.94 &  \textbf{91.84} &     \textbf{6.90} &      80.52 &  85.98 &     \textbf{5.47} &          \textbf{55.34} &  32.50 &   \textbf{-22.84} &          29.25 &  18.32 &   \textbf{-10.93} \\
        & \textbf{ctrst} &    - &  \textbf{93.76} &      - &       - &  91.28 &      - &        - &  \textbf{93.09} &      - &            - &  \textbf{29.12} &      - &            - &  \textbf{16.06} &      - \\
\midrule
\multirow{5}{*}{\textbf{OCSVM}} & \textbf{logits} &  51.71 &  59.31 &     \textbf{7.60} &     51.22 &  61.06 &     \textbf{9.84} &      51.36 &  57.29 &     \textbf{5.93} &          95.39 &  78.44 &   \textbf{-16.95} &          49.11 &  41.15 &    \textbf{-7.97} \\
        & \textbf{conv2x} &  57.65 &  57.45 &    -0.20 &     61.82 &  61.07 &    -0.74 &      73.69 &  72.69 &    -1.01 &          90.26 &  88.26 &    \textbf{-2.00} &          46.62 &  46.17 &    \textbf{-0.46} \\
        & \textbf{conv4x} &  63.44 &  64.52 &     \textbf{1.08} &     80.73 &  80.64 &    -0.09 &      78.76 &  79.12 &     \textbf{0.37} &          69.34 &  67.22 &    \textbf{-2.11} &          36.61 &  35.52 &    \textbf{-1.08} \\
        & \textbf{conv8x} &  \textbf{66.95} &  63.67 &    -3.28 &     \textbf{82.44} &  81.83 &    -0.60 &      \textbf{80.00} &  79.03 &    -0.98 &          \textbf{62.58} &  69.03 &     6.45 &          \textbf{33.10} &  36.33 &     3.23 \\
        & \textbf{ctrst} &    - &  \textbf{93.13} &      - &       - &  \textbf{92.67} &      - &        - &  \textbf{94.06} &      - &            - &  \textbf{25.98} &      - &            - &  \textbf{15.02} &      - \\
\midrule
\multirow{6}{*}{\textbf{RealNVP}} & \textbf{logits} &  80.52 &  76.22 &    -4.29 &     79.61 &  77.48 &    -2.12 &      79.82 &  73.18 &    -6.64 &          67.14 &  67.79 &     0.64 &          35.56 &  35.83 &     0.28 \\
        & \textbf{backbone} &  85.81 &  84.02 &    -1.79 &     90.13 &  89.09 &    -1.04 &      77.69 &  74.08 &    -3.61 &          31.17 &  32.49 &     1.31 &          17.49 &  18.18 &     0.69 \\
        & \textbf{conv2x} &  77.66 &  76.60 &    -1.06 &     75.72 &  76.39 &     \textbf{0.67} &      76.83 &  73.24 &    -3.59 &          70.63 &  71.81 &     1.18 &          37.33 &  37.73 &     0.40 \\
        & \textbf{conv4x} &  \textbf{92.30} &  91.79 &    -0.52 &     \textbf{92.84} &  92.93 &     \textbf{0.09} &      \textbf{90.32} &  88.48 &    -1.84 &          \textbf{27.39} &  34.80 &     7.42 &          \textbf{15.63} &  19.24 &     3.61 \\
        & \textbf{conv8x} &  90.10 &  87.13 &    -2.98 &     91.97 &  91.08 &    -0.89 &      85.62 &  80.26 &    -5.37 &          34.80 &  28.58 &    \textbf{-6.22} &          19.29 &  16.23 &    \textbf{-3.06} \\
        & \textbf{ctrst} &    - &  \textbf{94.79} &      - &       - &  \textbf{95.23} &      - &        - &  \textbf{92.62} &      - &            - &  \textbf{23.55} &      - &            - &  \textbf{13.62} &      - \\
\bottomrule
\end{tabular}
\caption{Results for KITTI ignored objects}
\label{tab:full_results_ignored}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{rc|ccc|ccc|ccc|ccc|ccc}
\toprule
        &       & \multicolumn{3}{c}{AUROC} & \multicolumn{3}{c}{AUPR (ID)} & \multicolumn{3}{c}{AUPR (OOD)} & \multicolumn{3}{c}{FPR @ 95\% TPR} & \multicolumn{3}{c}{Detection Err.} \\
       \textbf{OOD Method} &    \textbf{Layer}   &   Base &  Ctrst & $\Delta$ &      Base &  Ctrst & $\Delta$ &       Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ \\
\midrule
\textbf{Max Softmax} & \textbf{-} &  82.84 &  82.87 &     \textbf{0.03} &     88.06 &  88.36 &     \textbf{0.30} &      72.43 &  72.06 &    -0.37 &          36.41 &  34.05 &    \textbf{-2.36} &          20.64 &  19.40 &    \textbf{-1.23} \\
\textbf{Predictive Entropy} & \textbf{-} &  86.92 &  86.76 &    -0.16 &     90.83 &  90.93 &     \textbf{0.11} &      80.34 &  79.32 &    -1.02 &          29.69 &  27.96 &    \textbf{-1.73} &          17.22 &  16.23 &    \textbf{-0.99} \\
\textbf{Aleatoric Entropy} & \textbf{-} &  86.76 &  86.77 &     \textbf{0.02} &     90.69 &  90.90 &     \textbf{0.20} &      79.87 &  79.48 &    -0.39 &          30.09 &  28.24 &    \textbf{-1.86} &          17.44 &  16.37 &    \textbf{-1.07} \\
\textbf{Mutual Information} & \textbf{-} &  70.62 &  72.47 &     \textbf{1.86} &     66.79 &  69.55 &     \textbf{2.76} &      68.34 &  69.49 &     \textbf{1.15} &          85.78 &  82.66 &    \textbf{-3.12} &          45.37 &  43.82 &    \textbf{-1.55} \\
\midrule
\multirow{6}{*}{\textbf{Mahalanobis}} & \textbf{logits} &  47.34 &  49.66 &     \textbf{2.32} &     46.27 &  46.62 &     \textbf{0.34} &      52.99 &  55.72 &     \textbf{2.73} &          97.17 &  97.66 &     0.49 &          49.97 &  49.98 &     0.01 \\
        & \textbf{backbone} &  72.48 &  \textbf{80.60} &     \textbf{8.11} &     78.11 &  \textbf{86.52} &     \textbf{8.41} &      64.03 &  70.88 &     \textbf{6.85} &          59.52 &  \textbf{38.05} &   \textbf{-21.47} &          32.24 &  \textbf{21.43} &   \textbf{-10.80} \\
        & \textbf{conv2x} &  \textbf{76.18} &  79.94 &     \textbf{3.76} &     \textbf{81.64} &  85.00 &     \textbf{3.36} &      \textbf{67.34} & \textbf{ 72.18} &     \textbf{4.84} &          \textbf{53.12} &  44.72 &    \textbf{-8.40} &          \textbf{29.04} &  24.81 &    \textbf{-4.22} \\
        & \textbf{conv4x} &  47.69 &  55.70 &     \textbf{8.01} &     48.95 &  57.91 &     \textbf{8.96} &      47.58 &  51.88 &     \textbf{4.30} &          95.06 &  87.64 &    \textbf{-7.42} &          49.65 &  46.26 &    \textbf{-3.38} \\
        & \textbf{conv8x} &  42.91 &  51.91 &     \textbf{9.01} &     45.67 &  55.59 &     \textbf{9.92} &      44.45 &  49.29 &     \textbf{4.85} &          96.30 &  89.28 &    \textbf{-7.02} &          49.66 &  47.03 &    \textbf{-2.63} \\
        & \textbf{ctrst} &    &  50.02 &      - &       - &  52.86 &      - &        - &  49.30 &      - &            - &  90.70 &      - &            - &  46.57 &      - \\
\midrule
\multirow{5}{*}{\textbf{OC-SVM}} & \textbf{logits} &  54.72 &  35.60 &   -19.13 &     61.71 &  52.18 &    -9.53 &      63.23 &  50.06 &   -13.16 &          \textbf{67.89} &  \textbf{70.61} &     2.71 &          \textbf{34.76} &  \textbf{35.81} &     1.06 \\
        & \textbf{conv2x} &  54.35 &  57.45 &     \textbf{3.10} &     61.80 &  65.80 &     \textbf{4.00} &      70.37 &  72.34 &    \textbf{ 1.97} &          82.22 &  78.88 &    \textbf{-3.34} &          43.36 &  41.56 &    \textbf{-1.80} \\
        & \textbf{conv4x} &  23.16 &  24.00 &     \textbf{0.84} &     33.50 &  33.82 &     \textbf{0.33} &      46.59 &  47.40 &     \textbf{0.81} &          99.29 &  99.26 &    \textbf{-0.03} &          50.00 &  49.99 &    -0.00 \\
        & \textbf{conv8x} &  \textbf{63.22} &  \textbf{62.59} &    -0.63 &     \textbf{73.98} &  \textbf{79.64} &     \textbf{5.66} &      \textbf{77.07} &  \textbf{78.42} &     \textbf{1.35} &          72.03 &  70.91 &    \textbf{-1.11} &          38.34 &  37.48 &    \textbf{-0.87} \\
        & \textbf{ctrst} &    - &  10.30 &      - &       - &  32.18 &      - &        - &  32.49 &      - &            - &  99.40 &      - &            - &  50.00 &      - \\
\midrule
\multirow{6}{*}{\textbf{RealNVP}} & \textbf{logits} &  45.35 &  43.23 &    -2.11 &     48.57 &  48.00 &    -0.57 &      46.32 &  44.59 &    -1.73 &          94.23 &  94.18 &    \textbf{-0.05} &          48.17 &  48.88 &     0.71 \\
        & \textbf{backbone} &  \underline{\textbf{91.71}} &  \underline{\textbf{91.81}} &     \textbf{0.10} &     \underline{\textbf{94.69}} &  \underline{\textbf{94.79}} &     \textbf{0.09} &      \underline{\textbf{84.77}} &  \underline{\textbf{85.44}} &    \textbf{0.67} &          \underline{\textbf{16.25}} &  \underline{\textbf{15.44}} &    \textbf{-0.81} &           \underline{\textbf{9.58}} &   \underline{\textbf{8.99}} &    \textbf{-0.59} \\
        & \textbf{conv2x} &  60.67 &  77.25 &    \textbf{16.58} &     68.26 &  83.51 &    \textbf{15.25} &      57.28 &  68.29 &    \textbf{11.01} &          65.80 &  46.29 &   \textbf{-19.51} &          34.96 &  25.48 &    \textbf{-9.48} \\
        & \textbf{conv4x} &  70.46 &  74.13 &     \textbf{3.66} &     77.83 &  80.92 &     \textbf{3.09} &      62.13 &  65.78 &     \textbf{3.65} &          57.30 &  48.94 &    \textbf{-8.36} &          31.00 &  26.36 &    \textbf{-4.64} \\
        & \textbf{conv8x} &  77.71 &  78.96 &    \textbf{1.25} &     84.86 &  83.63 &    -1.23 &      66.30 &  71.48 &     \textbf{5.18} &          40.53 &  40.06 &    \textbf{-0.47} &          22.53 &  21.62 &    \textbf{-0.92} \\
        & \textbf{ctrst} &    - &  80.91 &      - &       - &  88.48 &      - &        - &  66.52 &      - &            - &  27.81 &      - &            - &  14.51 &      - \\
\bottomrule
\end{tabular}
\caption{Results for KITTI FP objects}
\label{tab:full_results_fp}
\end{table*}


\begin{table*}
\centering
\tiny
\begin{tabular}{rc|ccc|ccc|ccc|ccc|ccc}
\toprule
        &       & \multicolumn{3}{c}{AUROC} & \multicolumn{3}{c}{AUPR (ID)} & \multicolumn{3}{c}{AUPR (OOD)} & \multicolumn{3}{c}{FPR @ 95\% TPR} & \multicolumn{3}{c}{Detection Err.} \\
       \textbf{OOD Method} &    \textbf{Layer}   &   Base &  Ctrst & $\Delta$ &      Base &  Ctrst & $\Delta$ &       Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ &           Base &  Ctrst & $\Delta$ \\
\midrule
\textbf{Max Softmax} & \textbf{-} &  83.18 &  83.34 &     \textbf{0.16} &     85.41 &  86.51 &    \textbf{1.10} &      78.72 &  78.23 &    -0.49 &          52.17 &  45.80 &    \textbf{-6.36} &          28.53 &  25.35 &    \textbf{-3.18} \\
\textbf{Predictive Entropy} & \textbf{-} &  80.64 &  81.23 &     \textbf{0.58} &     83.86 &  85.29 &     \textbf{1.43} &      74.48 &  74.49 &     \textbf{0.01} &          53.69 &  47.50 &    \textbf{-6.19} &          29.29 &  26.19 &    \textbf{-3.10} \\
\textbf{Aleatoric Entropy} & \textbf{-} &  80.01 &  80.90 &     \textbf{0.88} &     83.45 &  85.05 &     \textbf{1.61} &      73.14 &  73.96 &     \textbf{0.82} &          53.97 &  47.62 &    \textbf{-6.36} &          29.44 &  26.27 &    \textbf{-3.17} \\
\textbf{Mutual Information} & \textbf{-} &  67.53 &  66.41 &    -1.12 &     63.31 &  63.70 &     \textbf{0.39} &      67.16 &  65.15 &    -2.01 &          90.14 &  86.23 &    \textbf{-3.91} &          47.50 &  45.56 &    \textbf{-1.93} \\
\midrule
\multirow{6}{*}{\textbf{Mahalanobis}} & \textbf{logits} &  52.45 &  52.37 &    -0.09 &     49.40 &  47.05 &    -2.36 &      58.55 &  62.28 &     \underline{\textbf{3.73}} &          96.29 &  98.21 &     1.93 &          49.73 &  49.98 &     0.25 \\
        & \textbf{backbone} &  \textbf{88.30} &  \textbf{82.21} &    -6.09 &     \textbf{88.59} &  \textbf{83.27} &    -5.32 &      \textbf{85.96} &  79.16 &    -6.80 &          \textbf{43.53} &  \textbf{51.34} &     7.80 &          \textbf{24.22} &  \textbf{28.11} &     3.89 \\
        & \textbf{conv2x} &  85.96 &  81.80 &    -4.16 &     85.04 &  80.29 &    -4.75 &      83.49 &  \textbf{79.77} &    -3.72 &          54.93 &  66.69 &    11.76 &          29.94 &  35.81 &     5.88 \\
        & \textbf{conv4x} &  73.61 &  69.04 &    -4.57 &     70.75 &  64.27 &    -6.48 &      72.48 &  69.60 &    -2.88 &          81.35 &  89.39 &     8.04 &          43.10 &  47.11 &     4.00 \\
        & \textbf{conv8x} &  69.90 &  71.70 &     \textbf{1.80} &     71.88 &  73.19 &     \textbf{1.31} &      63.76 &  65.78 &     \textbf{2.01} &          75.88 &  73.17 &    \textbf{-2.71} &          40.39 &  39.04 &    \textbf{-1.36} \\
        & \textbf{ctrst} &    - &  70.37 &      - &       - &  64.18 &      - &        - &  69.45 &      - &            - &  92.54 &      - &            - &  48.44 &      - \\
\midrule
\multirow{5}{*}{\textbf{OCSVM}} & \textbf{logits} &  48.13 &  55.08 &     \textbf{6.96} &     50.58 &  53.44 &     \textbf{2.86} &      47.96 &  56.23 &     \textbf{8.28} &          90.63 &  91.87 &     1.24 &          46.93 &  47.87 &     0.93 \\
        & \textbf{conv2x} &  63.66 &  64.51 &     \textbf{0.85} &     77.92 &  76.58 &    -1.34 &      \textbf{78.49} &  \textbf{78.42} &    -0.07 &          68.43 &  \textbf{66.47} &    \textbf{-1.96} &          36.33 &  \textbf{35.62} &    \textbf{-0.72} \\
        & \textbf{conv4x} &  62.36 &  62.95 &    \textbf{0.59} &     \textbf{78.15} &  76.19 &    -1.96 &      78.21 &  78.08 &    -0.13 &          71.18 &  69.82 &    \textbf{-1.36} &          37.65 &  37.27 &    \textbf{-0.39} \\
        & \textbf{conv8x} &  \textbf{64.74} &  62.20 &    -2.55 &     78.02 &  \textbf{78.00} &    -0.02 &      78.35 &  78.07 &    -0.28 &          \textbf{67.81} &  71.51 &     3.70 &          \textbf{36.17} &  37.94 &     1.77 \\
        & \textbf{ctrst} &    - &  \textbf{76.53} &      - &       - &  72.76 &      - &        - &  77.67 &      - &            - &  87.44 &      - &            - &  45.66 &      - \\
\midrule
\multirow{6}{*}{\textbf{RealNVP}} & \textbf{logits} &  59.93 &  55.35 &    -4.59 &     62.04 &  53.92 &    -8.12 &      57.74 &  54.51 &    -3.23 &          84.17 &  93.10 &     8.93 &          44.51 &  48.59 &     4.08 \\
        & \textbf{backbone} &  85.44 &  79.56 &    -5.88 &     89.46 &  84.60 &    -4.86 &      80.73 &  74.04 &    -6.69 &          33.03 &  46.01 &    12.98 &          18.92 &  25.43 &     6.51 \\
        & \textbf{conv2x} &  84.62 &  82.29 &    -2.33 &     85.65 &  83.18 &    -2.47 &      82.17 &  79.84 &    -2.34 &          51.38 &  57.98 &     6.61 &          28.14 &  31.46 &     3.32 \\
        & \textbf{conv4x} &  \underline{\textbf{91.45}} &  \underline{\textbf{88.93}} &    -2.53 &    \underline{\textbf{92.77}} &  \underline{\textbf{89.76}} &    -3.01 &      \underline{\textbf{88.86}} &  \underline{\textbf{86.86}} &    -2.00 &  \underline{\textbf{31.47}} &  \underline{\textbf{44.45}} &    12.98 &  \underline{\textbf{18.18}} &  \underline{\textbf{24.68}} &     6.50 \\
        & \textbf{conv8x} &  78.69 &  74.58 &    -4.10 &     82.43 &  79.87 &    -2.55 &      71.27 &  66.54 &    -4.74 &          54.13 &  56.44 &     2.30 &          29.52 &  30.67 &     1.15 \\
        & \textbf{ctrst} &    - &  79.28 &      - &       - &  79.32 &      - &        - &  74.74 &      - &            - &  65.70 &      - &            - &  35.31 &      - \\
\bottomrule
\end{tabular}
\caption{Results for Waymo objects}
\label{tab:full_results_waymo}
\end{table*}


==> tab/ignored_database.tex <==
\begin{table}
\centering
\scriptsize
\begin{tabular}{c|ccccc}
\toprule
Class &   Tram &  Truck & Van & Person sitting & Misc \\
\midrule
Quantity  & 287 &  606 & 1617 & 166 & 636\\
\bottomrule
\end{tabular}
\caption{The number of objects per class in  KITTI ignored OOD database}
\label{tab:ignored_database}
\end{table}


==> tab/object_statistics.tex <==
\begin{table*}
\centering
\tiny
\begin{tabular}{c|c|c|cccc|cccc|c}
\toprule
\multirow{3}{*}{Type} & \multirow{3}{*}{Class} & & \multicolumn{4}{c}{Base model} &  \multicolumn{4}{c}{Contrastive model} &
\\
&  & \# instances &
\# injection & \# detection & \# attempted & \# injected &
\# injection & \# detection & \# attempted & \# injected & 
\# common \\
& & in DB &
failures & failures & frames & objects &
failures & failures & frames & objects & 
OOD \\
\midrule
\multirow{5}{*}{Carla} 
 & ATM          & 10 & 17.51 &  43.52 & 545     & 300    & 16.20 & 40.25 & 489     & 300 & 289.67 \\ %262 & 309 & 298 \\
 & Bench        & 44 & 25.97 &  64.74 & 2342.67 & 289.33 & 22.61 & 55.70 & 1229.67 & 300 & 318.67 \\ %281 & 320 & 355 \\
 & Swing couch  & 25 & 29.37 &  60.96 & 2276.33 & 267.67 & 24.38 & 48.01 & 1631    & 300 & 200.67 \\ % 134 & 299 & 169 \\
 & Trash can 1  &  5 & 18.65 &  49.22 & 638.33  & 300    & 15.43 & 39.92 & 470.67  & 300 & 537.67 \\ % 549 & 542 & 522 \\
 & Trash can 2  &  5 & 4.02  &  9.38  & 304.67  & 300    & 2.39  & 5.40  & 302     & 300 & 582 \\ % 591 & 590 & 565 \\
\midrule
\multirow{4}{*}{KITTI Ignored} 
 & Tram             & 287 & - & - & - & - & - & - & - & - & 73.33 \\ % 67  & 60 & 105 \\
 & Truck            & 606 & - & - & - & - & - & - & - & - & 69.67 \\ % 68  & 72 & 69  \\
 & Person sitting   & 166 & - & - & - & - & - & - & - & - & 105.33 \\ % 106 & 114 & 96 \\
 & Misc             & 636 & - & - & - & - & - & - & - & - & 138 \\ % 139  & 152 & 123 \\
\midrule
\multirow{5}{*}{KITTI FP} 
 & Bike rack        & 11 & 0.71 & 0.04  & 300 & 300 & 0.93 & 0.09 & 300  & 300 & 599 \\ % 598  & 600 & 599 \\
 & Low traffic sign & 10 & 0.33 & 0.016 & 300 & 300 & 0.22 & 0.02 & 300  & 300 & 598.67 \\ % 597  & 599 & 600 \\
 & Sidewalk sign    & 33 & 0.57 & 0.008 & 300 & 300 & 0.37 & 0.02 & 300  & 300 & 599 \\ % 600 & 597 & 600 \\
 & Potted plant     & 9  & 0.89 & 0.03  & 300 & 300 & 0.69 & 0.03 & 300  & 300 & 599.33 \\ % 599 & 600 & 599 \\
 & Thin sign        & 3  & 0.54 & 0.084 & 300 & 300 & 0.36 & 0.06 & 300  & 300 & 598.67 \\ % 599 & 600 & 597 \\
\midrule
\multirow{4}{*}{Waymo}
 & Motorcycle   & 456 & 4.07 &  0.81 & 300    & 300 & 3.80  & 0.74 & 300    & 300 & 512 \\ % 519  & 502 & 515 \\
 & Scooter      & 80  & 9.68 &  1.39 & 300    & 300 & 8.18  & 1.01 & 300    & 300 & 385.67 \\ % 437 & 338 & 382 \\
 & Digger       & 49  & 4.57 &  1.03 & 300    & 300 & 4.48  & 1.00 & 300    & 300 & 585.67 \\ %588 & 583 & 586 \\
 &Excavator    & 44  & 13.35 &  3.04 & 302.33 & 300 & 11.67 & 2.65 & 300.33 & 300 & 564.33 \\ % 569  & 549 & 575 \\
\bottomrule
\end{tabular}
\caption{Statistics for OOD objects. In total, we generate six datasets, one for each model/seed combination. The injection statistics (\# injection failures, \# detection failures, \# attempted frames, \# injected objects) and \# common OOD are averaged over three seeds. }
\label{tab:object_statistics}
\end{table*}




%%%%%%%Base
% Atm
% [ 17.51  43.52 545.        ]
% Bench01
% [  25.97   64.74 2342.66]
% SwingCouch
% [  29.37   60.96 2276.33]
% TrashCan01
% [ 18.65  49.22 638.33]
% TrashCan02
% [  4.02    9.38 304.66]

% bike_rack
% [  0.71   0.04 300.   ]
% low_traffic_sign
% [  0.33   0.016 300.   ]
% sidewalk_sign
% [  0.57    0.01 300.   ]
% potted_plant
% [  0.89   0.03 300.   ]
% thin_sign
% [  0.54    0.08 300.   ]

% motorcycle
% [  4.07   0.81 300.        ]
% scooter
% [  9.68   1.39 300.        ]
% digger
% [  4.57   1.03 300.        ]
% excavator
% [ 13.35   3.04 302.33]




%%%%%%%%Contrastive
% Atm
% [ 16.20 40.25  489.0        ]
% Bench01
% [ 22.61 55.70 1229.66]
% SwingCouch
% [ 24.38 48.01 1631.0        ]
% TrashCan01
% [ 15.43 39.92 470.66]
% TrashCan02
% [  2.39 5.40 302.0        ]

% bike rack
% [  0.93   0.09  300.   ]
% low_traffic_sign
% [  0.22   0.02 300.   ]
% sidewalk_sign
% [  0.37   0.02  300.   ]
% potted_plant
% [  0.69   0.03 300.   ]
% thin_sign
% [  0.36   0.06 300.   ]

% motorcycle
% [  3.80 0.74 300.        ]
% scooter
% [  8.18 1.01 300.        ]
% digger
% [  4.48 1.0 300.        ]
% excavator
% [ 11.67 2.65 300.33]




==> tab/ood_cat.tex <==
\begin{table}
\centering
\resizebox{.65\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccc@{}}
\toprule
 & \textbf{Class} & \textbf{In train dist ?} & \textbf{Detected} \\
\hline
1 & FG & \checkmark & \checkmark  \\
\hline
2& FG & \checkmark & \xmark
\\
\hline
3 & FG & \xmark & \checkmark  \\
\hline
4 & FG & \xmark &  \xmark\\
\hline
5 & BG & \checkmark & \checkmark \\
\hline
6 & BG & \checkmark & \xmark \\
\hline
7 & BG & \xmark & \checkmark\\
\hline
8 & BG & \xmark & \xmark\\
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
OOD categorisation
% 
} % \caption
\label{tab:ood_cat}
\end{table}

==> tab/ood_dataset_uncertainty.tex <==
\begin{table}
\centering
\resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
\begin{tabular}{@{}lccccc@{}}
\toprule
Uncertainty & \textbf{KITTI ignored} & \textbf{Carla} & \textbf{Waymo} & \textbf{KITTI FP} & \textbf{All} \\
\hline
Aleatoric & 60\%   & 75 \%  & 80 \% & 92\% & 84 \%   \\
\hline
Espitemic & 40 \%  & 20 \%  & 10 \% & 5 \% & 10 \% \\ 
\bottomrule
\end{tabular}
} %< \resizebox
\caption{
% 
Uncertainty in our generated OOD dataset. Table shows percentage of objects with aleatoric uncertainty $> 0.5$ and percentage objects with espitemic uncertainty $> 0.01$
% 
} % \caption
\label{tab:ood_dataset_uncertainty}
\end{table}

==> tab/waymo_adding_statistics.tex <==
\begin{table}
\centering
\tiny
\begin{tabular}{c|ccc}
\toprule
Class & Adding failures & Detecting failures & Number of attempted frames \\
\midrule
Motorcycle  & 3.93 &  0.77 & 300 \\
\midrule
Scooter  & 8.93 &  1.20 & 300       \\
\midrule
Digger  & 4.53 & 1.02 & 300 \\
\midrule
Excavator & 12.51 &  2.85 & 301   \\
\bottomrule
\end{tabular}
\caption{Waymo inserting statistics}
\label{tab:waymo_inserting_statistics}
\end{table}

% motorcycle
% [  3.93555556   0.77666667 300.        ]
% scooter
% [  8.93722222   1.20388889 300.        ]
% digger
% [  4.53         1.02166667 300.        ]
% excavator
% [ 12.51193959   2.85008623 301.33333333]

==> tab/waymo_database.tex <==
\begin{table}
\centering
\scriptsize
\begin{tabular}{c|cccc}
\toprule
Class &   Motorcycle &  Scooter & Digger & Excavator \\
\midrule
Quantity  & 456 &  80 & 49 & 44\\
\bottomrule
\end{tabular}
\caption{The number of objects per selected class in  Waymo OOD database}
\label{tab:waymo_database}
\end{table}
